Algorithms and Bounds for Drawing Non-planar Graphs with Crossing-free Subgraphs

We initiate the study of the following problem: Given a non-planar graph G and a planar subgraph S of G, does there exist a straight-line drawing {\Gamma} of G in the plane such that the edges of S are not crossed in {\Gamma} by any edge of G? We give positive and negative results for different kinds of connected spanning subgraphs S of G. Moreover, in order to enlarge the subset of instances that admit a solution, we consider the possibility of bending the edges of G not in S; in this setting we discuss different trade-offs between the number of bends and the required drawing area.

==> makefile <==
finalname = main

pdf: $(finalname)


included_latex_sources = 

latex_compiler=pdflatex
#latex_compiler=pdflatex

#psfiles = \


# pdf: $(finalname)
# 	dvips -Ppdf $(finalname).dvi -o $(finalname).ps
# 	ps2pdf $(finalname).ps $(finalname).pdf

bib: 
	$(latex_compiler) $(finalname).tex
	bibtex $(finalname)
	$(latex_compiler) $(finalname).tex
	$(latex_compiler) $(finalname).tex

$(finalname): $(included_latex_sources) $(psfiles) $(finalname).tex
	$(latex_compiler) $(finalname).tex 

%.ps: %.fig
	fig2dev -Leps $< $@

%.ps: %.gif
	convert $< $@

%.ps: %.bmp
	convert $< $@

%.ps: %.jpg
	convert $< $@

clean:
	rm -f $(psfiles)
	rm -f $(finalname).ps
	rm -f tmp-data/*.avg
	rm -f tmp-data/*.txt
	rm -f src-data/*.tmp
	rm -f *~
	rm -f *.bak
	rm -f figures/*.bak
	rm -f *.toc
	rm -f *.aux
	rm -f *.blg
	rm -f *.dvi
	rm -f *.log
	rm -f *.out
	rm -f *.bbl
	rm -f *.backup


ps: $(finalname)
	dvips -t a4 $(finalname).dvi -o # -pp 6 -t a4

#	dvips -t letter $(finalname).dvi -o


print: ps
	lpr -Ppolaris -h $(finalname).ps

